Identifying and Exploiting Structures for Reliable Deep Learning

Deep learning research has recently witnessed an impressively fast-paced progress in a wide range of tasks including computer vision, natural language processing, and reinforcement learning. The extraordinary performance of these systems often gives the impression that they can be used to revolutionise our lives for the better. However, as recent works point out, these systems suffer from several issues that make them unreliable for use in the real world, including vulnerability to adversarial attacks (Szegedy et al. [248]), tendency to memorise noise (Zhang et al. [292]), being over-confident on incorrect predictions (miscalibration) (Guo et al. [99]), and unsuitability for handling private data (Gilad-Bachrach et al. [88]). In this thesis, we look at each of these issues in detail, investigate their causes, and propose computationally cheap algorithms for mitigating them in practice. To do this, we identify structures in deep neural networks that can be exploited to mitigate the above causes of unreliability of deep learning algorithms.

==> adv_cause_folder/__latexindent_temp.tex <==
\section{Experimental results on the impact of memorising label noise}
\label{sec:exp-overfit-mislbl}

This section will look at empirical results on synthetic data, inspired
by the theory and on the standard datasets: MNIST~\citep{LBBH:1998} and
CIFAR10~\citep{krizhevsky2009learning}, that shows the impact of memorising label noise on adversarial vulnerability.
\subsection{Memorisation of label noise hurts adversarial accuracy}
\paragraph{Experiments on toy-MNIST}
We design a simple binary classification problem, \emph{toy-MNIST}, and show
that when fitting a complex classifier on a training dataset with label noise,
adversarial vulnerability increases with the amount of label noise and that this
vulnerability is caused by the label noise. The problem is constructed by
selecting two images from MNIST: one ``0'' and one ``1''. Each training/test
example is generated by selecting one of these images and adding i.i.d. Gaussian
noise sampled from $\cN\br{0,\sigma^2}$ for some \(\sigma>0\). We create a
training dataset of $4000$ samples by sampling uniformly from either class.
Finally, $\eta$ fraction of the training data is chosen randomly and its labels
are flipped. 
We train a neural network with four fully connected layers followed by a softmax
layer and minimise the cross-entropy loss using an SGD optimiser until the
training error becomes zero. Then, we attack this network with a ~\emph{strong}
$\ell_\infty$ PGD adversary~(discussed
in~\Cref{sec:adv-attack-bg})~\citep{madry2018towards} with
$\epsilon=\frac{64}{255}$ for $400$ steps with a step size of $0.01$. 

\begin{figure}[t]
    \begin{subfigure}[t]{0.49\linewidth}
      \begin{subfigure}[t]{0.32\linewidth}
      \centering
      \def\svgwidth{0.99\columnwidth}
      \input{./adv_cause_folder/figures/error_vs_random_01.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.32\linewidth}
        \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/error_vs_random_03.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.32\linewidth}
        \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/error_vs_random_05.pdf_tex}
      \end{subfigure}
    \caption{Toy-MNIST , $\epsilon=\frac{64}{255}$}
    \label{fig:risk_vs_noise}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.49\linewidth}
      \begin{subfigure}[t]{0.32\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/001_20_mnist_mis_adv_risk.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.32\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/005_20_mnist_mis_adv_risk.pdf_tex}
      \end{subfigure}
       \begin{subfigure}[t]{0.32\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/01_20_mnist_mis_adv_risk.pdf_tex}
      \end{subfigure}
      \caption{Full-MNIST}
      \label{fig:mnist_lbl_noise_adv}
    \end{subfigure}\vspace{10pt}
      \begin{subfigure}[t]{0.99\linewidth}
      \begin{subfigure}[t]{0.32\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/R18_adv_noise.pdf_tex}
        \caption{ResNet18~(CIFAR10)}
      \label{fig:risk_vs_noise_cifar10_r18}
      \end{subfigure}
      \begin{subfigure}[t]{0.33\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/D121_adv_noise.pdf_tex}
        \caption{DenseNet121~(CIFAR10)}
      \label{fig:risk_vs_noise_cifar10_d121}
      \end{subfigure}
      \begin{subfigure}[t]{0.32\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/VGG19_adv_noise.pdf_tex}
        \caption{VGG19~(CIFAR10)}
        \label{fig:risk_vs_noise_cifar10_vgg}
      \end{subfigure}
    \end{subfigure}
    \caption[Adversarial error increases with label noise]{Adversarial Error
    increases with increasing label noise~$\eta$.  The shaded region indicates a
    $95\%$ confidence interval. The absence of a shaded region indicates that it
    is invisible due to low variance.}
    
  \end{figure}
  
In~\Cref{fig:risk_vs_noise}, we plot the adversarial error, natural test error
and training error as the amount of label noise $(\eta)$ varies, for three
different values of sample variance~($\sigma^2$). For low values of
$\sigma^2$~($\sigma^2=0.1$), the training data from each class are all
concentrated around the same point; as a result, these models are unable to
memorise the label noise and the training error is high. In this case,
over-fitting label noise is impossible and the test error, as well as the
adversarial error, is low. This does not contradict~\Cref{thm:inf-label}, which
requires zero training error on the mislabelled dataset. However, as $\sigma^2$
increases to~$\sigma^2=0.5$, the neural network is flexible enough to use the
``noise component'' to extract features\todo[color=red]{Can we prove it or show evidence in support of this ?} that allow it to memorise label noise
and fit the training data perfectly. This brings the training error down to
zero while causing the test error to increase, and the adversarial error even
more so. This is in line with Theorem~\ref{thm:inf-label}. \begin{remark} The
case when $\sigma^2=0.3$ is particularly interesting; when the label noise is
low and the training error is high, there is no overfitting and the test error
and the adversarial error is zero. When the network starts memorising label
noise~(i.e. train error gets lesser than label noise), test error remains
very low  but adversarial error increases rapidly. \end{remark}

\paragraph{Experiments on the full MNIST and CIFAR10 dataset}
We perform a similar experiment on the full MNIST dataset trained on a 4-layered
Convolutional Neural Network. The model architecture consists of four
convolutional layers, followed by two fully connected layers. The first four
convolutional layers have $32,64, 128$, and  $256$ output filters with kernels of width $3,4,3,$ and $3$ respectively. The two fully connected
layers have a width of $1024$. The network is optimised with SGD with a batch
size of $128$ and an initial learning rate of $0.1$ for a total of $60$ epochs.
The learning rate is decreased to $0.01$ after $50$ epochs.  For varying values
of $\eta$, we assign a uniformly randomly label to a randomly chosen $\eta$
fraction of the training data.  We compute the natural test accuracy and the
adversarial test accuracy on a clean test-set with no label noise for when the
network is attacked with an $\ell_\infty$ bounded PGD adversary for varying
perturbation budget $\epsilon$, with a step size of $0.01$ and for $20$ steps
and plot the results in~\Cref{fig:mnist_lbl_noise_adv}.  We repeat the same
experiment for CIFAR10 with a DenseNet121~\citep{HZWV:2017},
ResNet18~\citep{HZRS:2016}, and VGG19~\citep{simonyan2014very}  to test the
phenomenon across multiple state-of-the-art architectures and plot the results
in~\Cref{fig:risk_vs_noise_cifar10_r18,fig:risk_vs_noise_cifar10_d121,fig:risk_vs_noise_cifar10_vgg}.
Please refer to~\Cref{sec:expr-settings} for more details on the architectures
and datasets. The results on both datasets show that the effect of over-fitting
label noise on adversarial error is even more clearly  visible here; for the
same PGD adversary, the adversarial error jumps upwards sharply with increasing
label noise, while the growth of natural test error is much slower. This
confirms the hypothesis that benign overfitting may not be so benign when it
comes to adversarial error.

\subsection{Representations of label noise and adversarial examples}

For the toy-MNIST problem, we plot a 2-d projection~(using PCA) of the learned
representations~(activations before the last layer) at various stages of
training in~\Cref{fig:represen}. We remark that the simplicity of the data model
ensures that even a 1-d PCA projection suffices to perfectly separate the
classes when there is no label noise; however, the representations learned by a
neural network in the presence of noise may be very different! We highlight two
key observations: 
\begin{figure}[t]
  \begin{subfigure}[t]{0.15\linewidth}
    \centering \def\svgwidth{0.99\columnwidth}
    \input{./adv_cause_folder/figures/legend_representation.pdf_tex}
  \end{subfigure}\hfill
                 \begin{subfigure}[t]{0.8\linewidth}
    \centering \def\svgwidth{0.99\columnwidth}
    \input{./adv_cause_folder/figures/representation.pdf_tex}
  \end{subfigure}
  \caption[Representation of mislabelled and adversarial examples]{Two dimensional PCA projections of the original correctly
    labelled~(blue and orange), original mislabelled~(green and red),
    and adversarial examples~(purple and brown) at different stages of
    training. The correct label for~\emph{True 0}~(blue),~\emph{Noisy 0}~(green),~\emph{Adv
    0}~(purple +) are the same i.e. 0 and similar for the other class.}
  \label{fig:represen}
\end{figure} 


\begin{enumerate}
  \item   The bulk of adversarial examples~(``$+$''-es) are
concentrated around the mislabeled training data~(``$\circ$''-es) of the
opposite class. For example, the purple $+$-es~(Adversarially
perturbed: True: 0, Pred:1 ) are very close to the green
$\circ$-es~(Mislabelled: True:0, Pred: 1). This provides empirical
validation for the  hypothesis that if
there is a mislabeled data point in the vicinity that has been fit by the
model, an adversarial example is created by moving towards that data point
as predicted by~\Cref{thm:inf-label}. 
\item   The mislabeled training data take longer to be fit by the classifier.
For example, by iteration 20, the network learns a fairly good representation
and classification boundary that correctly fits the clean training data (but not
the noisy training data). At this stage, the number of adversarial examples is
much lower as compared to Iteration 160, by which point the network has
completely fit the noisy training data. Thus early stopping helps in avoiding
\emph{memorising} the label noise, and consequently also reduces adversarial
vulnerability. Early stopping has indeed been used as a defence in quite a few
recent papers in the context of adversarial
robustness~\citep{Wong2020Fast,hendrycks2019pretraining}, as well as learning in
the presence of label-noise~\citep{Li2019}. Our work shows \emph{why} early
stopping may reduce adversarial vulnerability by avoiding fitting noisy training
data.  
\end{enumerate}

\subsection{Robust training avoids memorisation of rare examples}
\label{sec:robust-avoid-mem}

Robust training methods like AT~\citep{madry2018towards} and
TRADES~\citep{Zhang2019} are commonly used data-augmentation based techniques to
increase the adversarial robustness of deep neural networks. However, it has been
pointed out that this comes at a cost to clean
accuracy~\citep{Raghunathan2019,tsipras2018robustness}. When trained with these
methods, both the training and test accuracy (on clean data) for commonly used
deep learning models drops with increasing strength of the PGD adversary used in
the adversarial training~(see~\Cref{tab:accs-robust-models}). In this section, we
provide  evidence to show that robust training avoids memorisation of label
noise and this also results in the drop of clean train and test accuracy. Before
going further, we will first describe how we measure memorisation and related
concepts. We borrow these two concepts from~\citet{Zhang2020} who measure the
label memorisation phenomenon using two related measures: {\em memorisation} and
{\em influence}. 

\begin{table}[t]
  \centering
  \begin{tabular}{|ccc|}\toprule
    $\epsilon$&Train-Acc.~($\%$)&Test-Acc~($\%$)\\\midrule
    0.0&99.98&95.25\\
    0.25&97.23&92.77\\
    1.0&86.03&81.62\\\bottomrule
  \end{tabular}
   \caption[Robust Training decreases clean train and test
    accuracies]{Train and Test Accuracies on Clean Dataset for
    ResNet-50 models trained using $\ell_2$ adversaries}
  \label{tab:accs-robust-models}
\end{table}

\paragraph{Memorisation or Self-Influence:} Self influence of an example
$\br{\vec{x}_i,y_i}$ for a dataset $\cS$ and learning algorithm
$\cA$~(including model, optimiser etc) can be defined as how unlikely it is for
the model learnt by $\cA$ to be correct on $\br{\vec{x}_i,y_i}$ if the training
dataset $\cS$ does not contain $\br{\vec{x}_i,y_i}$ compared to if $\cS$
contains $\br{\vec{x}_i,y_i}$. It can be formalised as follows which is
borrowed from Eq~(1) in~\citet{Zhang2020}

Memorisation by $\cA$ on example $(x_i,y_i) \in \cS$ is measured as
\[{\mathrm{mem}(\cA,\cS,i) := \bP_{h\sim \cA(\cS)}[h(x_i) = y_i] -
\bP_{h\sim \cA(\cS^{\setminus i})}[h(x_i) = y_i]}\]

where $\cS^{\setminus i}$ denotes the dataset $\cS$ with $(x_i,y_i)$ removed,
$h\sim \cA(\cS)$ denotes the model $h$ obtained by training using
algorithm $\cA$~(which includes the model architecture) on the dataset $\cS$ and
the probability is taken over the randomisation inherent in the training
algorithm $\cA$.

\paragraph{Influence of a training example on a test example:} Given a training
example $\br{\vec{x}_i, y_i}$, a test example $\br{\vec{x}'_j,y'_j}$, a training
dataset $\cS$ and a learning algorithm $\cA$, the influence of  $\br{\vec{x}_i,
y_i}$ on $\br{\vec{x}'_j,y'_j}$ measures the  probability that
$\br{\vec{x}'_j,y'_j}$ would be classified correctly if the training set $\cS$
does not contain  $\br{\vec{x}_i, y_i}$ compared to if it does. This can be
defined as follows which is borrowed from Eq 2 in~\citet{Zhang2020}. Using a
similar notation as memorisation, the influence of $(x_i, y_i)$ on $(x'_j,y'_j)$
for the learning algorithm $\cA$ with training dataset $\cS$ can be measured as

\[\mathrm{infl}(\cA,\cS,(x_i,y_i),(x'_j,y'_j)) := \bP_{h\sim
\cA(\cS)}[h(x'_j) = y'_j] - 
\bP_{h\sim \cA(\cS^{\setminus i})}[h(x'_j) = y'_j]\] 



\paragraph{Robust training ignores label noise}
~\Cref{fig:mislabelled_ds} shows that label noise is not uncommon in standard
datasets like MNIST and CIFAR10. In fact, upon closely monitoring the
misclassified training set examples for both~\AT and TRADES, we found that
neither AT nor TRADES predicts correctly on the training set labels for any of
the examples identified in~\Cref{fig:mislabelled_ds}, all examples that have a
wrong label in the training set, whereas natural  training does. Thus, in line
with~\Cref{thm:inf-label}, robust training methods ignore fitting noisy labels.

We also observe this in a synthetic experiment on the full MNIST dataset where
we assigned random labels to 15\% of the dataset. A naturally trained CNN model
achieved $100\%$ train accuracy on this dataset whereas an adversarially trained
model~(standard setting with $\epsilon=0.3$ for $30$ steps) misclassified $997$
examples in the training set after the same training regime. Out of these $997$
samples, $994$ examples belonged to that \(15\%\) of the examples that were
mislabelled in the dataset.


\paragraph{Robust training ignores rare examples}
Certain examples in the training set belong to rare sub-populations~(eg. a
special kind of cat) and this sub-population is sufficiently distinct from the
rest of the examples of that class in the training dataset~(other cats in the
dataset). Next, we show that though ignoring rare samples possibly helps in
adversarial robustness, it hurts the natural test accuracy. We hypothesise
that one of the effects of robust training is to not \emph{memorise rare
examples}, which would otherwise be memorised by a naturally trained model.
As~\citet{Feldman2019} points out,\emph{ if these sub-populations are very
infrequent in the training dataset, they are indistinguishable from data points
with label noise with the difference being that examples from that
sub-population are also present in the test-set}. Natural training by
\emph{memorising} those rare training examples reduces the test error on the
corresponding test examples. Robust training, by not memorising these rare
samples~(and label noise), achieves better robustness but sacrifices the test
accuracy on the test examples corresponding to those  training points.
\paragraph{Experiments on MNIST, CIFAR10, and ImageNet} We visually demonstrate
this effect in~\Cref{fig:adv-train-test-mis-class} with examples from CIFAR10,
MNIST, and ImageNet and then provide more statistical evidence using the notions
of memorisation score and influence~\citep{Zhang2020}
in~\Cref{fig:infl-cifar10-mem}. Each pair of images contains a
misclassified~(by robustly trained models) test image and the misclassified
training image ``responsible'' for it.
Importantly both of
these images were correctly classified by a naturally trained
model. Visually, it is evident that the training images are  
extremely similar to the corresponding test image.  Inspecting the
rest of the training set, they are also very different from other
images in the training set. We can thus refer to these as rare
sub-populations. 

We found the images in~\Cref{fig:adv-train-test-mis-class} by manually searching
for each test  image, the training image that is misclassified and is visually
close to it. Our search space was shortened with the help of the influence
scores of each training image on the test image. We searched in the set of
top-$10$ most influential misclassified train images for each misclassified
test image. The model used for~\cref{fig:adv-train-test-mis-class} is a) an \AT
ResNet50 model for  CIFAR10 with $\ell_2$-adversary with an $\epsilon=0.25$, b)
a model trained with TRADES for MNIST with $\lambda=\frac{1}{6}$ and
$\epsilon=0.3$, and c) and \AT ResNet50 model for Imagenet with $\ell_2$
adversary with $\epsilon=3.0$. ~\citet{Zhang2020}  provided us the with the
memorisation scores for each image in CIFAR10 as well as the influence score of
each training image on each test image for each class in CIFAR-10. High
Influence pairs of Imagenet were obtained
from~\url{https://pluskid.github.io/influence-memorization/}. This was used to
obtain the figures for the Imagenet dataset
in~\Cref{fig:adv-train-test-mis-class}. 

\begin{figure}[t]
    \centering
   \begin{subfigure}[b]{0.53\linewidth}
   \begin{subfigure}[t]{0.99\linewidth}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/ostrich.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/water_birds.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/wheat_bird.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/cat_eye.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.99\linewidth}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/b54.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/wheel_truck.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/red_truck.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/eye_deer.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.99\linewidth}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/yellow_cat.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/boeing.png}
      \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/green_wall_cat.png}
  \includegraphics[width=0.24\linewidth]{./adv_cause_folder/figures/adv_mis_tr_te/water_deer.png}
  \end{subfigure}
  \caption*{CIFAR10}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\linewidth}
    \centering \def\svgwidth{0.99\linewidth}
    \input{./adv_cause_folder/figures/adv_mis_tr_te_mnist.pdf_tex}
    \caption*{MNIST}
  \end{subfigure}
  
    \begin{subfigure}[b]{0.99\linewidth}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_1_lbl_6_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_82_lbl_199_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_161_lbl_419_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_173_lbl_439_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_193_lbl_480_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_207_lbl_506_cropped.pdf_tex}
      \end{subfigure}
    \end{subfigure}
    \begin{subfigure}[b]{0.99\linewidth}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_404_lbl_823_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_411_lbl_828_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_444_lbl_859_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_441_lbl_855_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_304_lbl_697_cropped.pdf_tex}
      \end{subfigure}
      \begin{subfigure}[t]{0.16\linewidth}
        \centering \def\svgwidth{0.99\columnwidth}
        \input{./adv_cause_folder/figures/imagenet_high_inf/high_infl_346_lbl_751_cropped.pdf_tex}
      \end{subfigure}
      \caption*{ImageNet}
    \end{subfigure}
  \caption[Adversarial Training Ignores High Influence Train-test Pairs]{Each pair is a  training~(left)
      and  test~(right) image misclassified by the adversarially
      trained model. They were both correctly classified
      by the naturally-trained model.}
    \label{fig:adv-train-test-mis-class}
  \end{figure}

  A precise notion of
  measuring if a sample is~\emph{rare} is through the concept of
  self-influence or memorisation. Self-influence for a~\emph{rare
  example}, that is unlike other examples of that class, will be high as
  the rest of the dataset will \emph{not} provide relevant information
  that will help the model to  
  correctly predict on that particular example.
  In~\cref{fig:cifar_self_influence}, we show that the self-influence of
  training samples that were misclassified by adversarially trained models but
  correctly classified by a naturally trained model is higher  compared to the
  distribution of self-influence on the entire train dataset. In other words, it
  means that the  self-influence  of the training examples misclassified by the
  robustly trained models is larger than the average self-influence of ~(all)
  examples belonging to that class. This supports our hypothesis that
  adversarial training excludes fitting these rare~(or ones that need to be
  memorised) samples.


The notion that certain test examples were not classified correctly due to a particular training example not being classified correctly is measured by the
\emph{influence} a training image has on the test image~(c.f. definition 3
in~\citet{Zhang2020}). We obtained the influence of each training image on each
test image for that class from~\citet{Zhang2020} and the training images in
~\Cref{fig:adv-train-test-mis-class} has a disproportionately higher influence
on the corresponding test image compared to influences of other train-test image
pairs in CIFAR10.  

In ~\Cref{fig:infl-cifar10_tr_te_adv}, we show that the influence of training
images are higher on test images that are misclassified by adversarially
trained models as compared to an average test image from the dataset. In other
words, this means that adversarially trained models misclassify test examples
that are being heavily influenced by some particular training example. As we saw
in~\Cref{fig:cifar_self_influence},  AT models do not memorise atypical train
examples; consequently, they misclassify test examples that are heavily
influenced by those atypical train examples~(visualised
in~\Cref{fig:adv-train-test-mis-class}).  This confirms our hypothesis that the
loss in test accuracy of robustly trained models is due to test images that
are~\emph{rare} and thus have a particularly high influence from a training
image.


\begin{figure}[t]
    \begin{subfigure}[b]{0.7\linewidth}
    \begin{subfigure}[t]{0.99\linewidth}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_plane.pdf_tex}
        \caption*{PLANES}    
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_car.pdf_tex}
        \caption*{CAR}     
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_bird.pdf_tex}
        \caption*{BIRD}     
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_cat.pdf_tex}
        \caption*{CAT}    
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_deer.pdf_tex}
        \caption*{DEER}     
      \end{subfigure}
    \end{subfigure}
      \begin{subfigure}[t]{1.0\linewidth}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_dog.pdf_tex}
        \caption*{DOG}      
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_frog.pdf_tex}
        \caption*{FROG}      
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_horse.pdf_tex}
        \caption*{HORSE}     
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_ship.pdf_tex}
        \caption*{SHIP}
      \end{subfigure}
      \begin{subfigure}[t]{0.19\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./adv_cause_folder/figures/self_influence_truck.pdf_tex}
        \caption*{TRUCK}
      \end{subfigure}
    \end{subfigure}
    \caption{Fraction of train points that have a
      self-influence greater than $s$ is plotted versus $s$. }
  \label{fig:cifar_self_influence}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.29\linewidth}
    \centering \def\svgwidth{0.99\linewidth}
    \input{./adv_cause_folder/figures/adv_train_test_infl.pdf_tex}
    \caption{Distribution of the influence of training point  on 
    all test points compared to the distribution of influence on test
    points mis-classified by adversarially trained points. }
    \label{fig:infl-cifar10_tr_te_adv}
  \end{subfigure}
  \caption[Adversarial
  training ignores high training points with high self-influence]{The blue represents the points misclassified by an
  adversarially trained model. The orange represents the distribution
  for all points in the dataset~(of the concerned class for CIFAR10).
  }
  \label{fig:infl-cifar10-mem}
  \end{figure}
  
\begin{remark}\todo[color=green]{Comment how any method that does not memorise will suffer from this}
We remark that this behaviour of \AT and TRADES seemingly induces a tradeoff
between natural test error and adversarial error in the presence of label noise.
However, this is under the assumption that the learning algorithm cannot
distinguish between examples with label noise and atypical examples. Our
experiments indicate that \AT and TRADES is unable to distinguish between them.
However, if an algorithm can distinguish between them then this
specific kind of tradeoff should not arise although there might still be
tradeoffs for other reasons.

This drop in test accuracy due to not memorising rare or atypical samples is not
specific to \AT and TRADES but seen in other learning algorithms, that avoid
memorisation, as well. In particular, this has been observed in differentially
private training~\citep{bagdasaryan19} and sparse training~\citep{hooker2019compressed} as well.\todo[color=green]{COmplete
this citation}
\end{remark}

==> low_rank_folder/__latexindent_temp.tex <==
\label{sec:what-low-rank}
Consider $f: \mathbb{R}^d \mapsto \mathbb{R}^k$ to be a feed-forward MLP that
maps $d$ dimensional input $\vx$ to a $k$ dimensional output $\vy$. We can
decompose this into two sub-networks, one consisting of the layers before the
$\ell^{\it th}$ layer and one after i.e.  $f(\vx) =
f^{+}_\ell\br{f^{-}_\ell(\vx; \phi) ; \theta}$, where $f^{-}_\ell (.;\phi)$,
parameterised by $\phi$, represents the part of the network up to layer $\ell$
and, $f^{+}_\ell(.;\theta)$ represents the part of the network thereafter. With
this notation, the $m$ dimensional representation (or the activations) after
any layer $\ell$ can simply be written as $\va = f^{-}_\ell(\vx; \phi) \in
\mathbb{R}^m$. In what follows, we first formalise the low-rank representation
problem and then propose our approach to solve it approximately and efficiently.

\subsection{Formulating the LR Layer problem} Let $\vec{X} = \{\vec{x}_i\}_{i=1}^N$
and $\vec{Y} = \{{\bf y}_i\}_{i=1}^N$ be the set of inputs and target outputs of
a given training dataset. By slight abuse of notation, we define $\vec{A}_\ell =
f^{-}_\ell(\vec{X}; \phi) =\bs{\vec{a}_1,\cdots,\vec{a}_N}^\top\in \mathbb{R}^{N
\times m}$ to be the activation matrix of the entire dataset, so that
$\vec{a}_i$ is the activation vector of the $i$-th sample. Note that for most
practical purposes $N\gg m$. In this setting, the problem of learning low-rank
representations can be formulated as a constrained optimisation problem as
follows:
\begin{align}
  \label{eq:opt_prob}
	\min_{\theta, \phi}\mathcal{L}(\vec{X}, \vec{Y}; \theta, 
  \phi),~\text{s.t.}~~&\rank{\vec{A}_\ell} = r,\end{align} 
where $\mathcal{L}(.)$ is the loss function and $r < m$ is the desired rank of
the representations at layer $\ell$. The rank $r$ is a hyperparameter (though
empirically not a sensitive one as observed in our experiments). Throughout this
section, we discuss the problem of imposing low-rank constraints over a single
intermediate layer, however, it can trivially be extended to any number of
layers. Note that both the loss and the constraint set of the above objective
function are non-convex. One approach to optimising this would be to perform an
alternate minimisation style algorithm~(eg.~\citep{Lloyd1982,Dempster1977}),
first over the loss (gradient descent) and then projecting onto the non-convex
set to satisfy the rank constraint.

Since $N \gg m$, ensuring $\rank{\vec{A}_\ell} = r$ would  be practically
infeasible as it would require performing SVD in every iteration at a cost
$\mathcal{O}(N^2m)$. A feasible, but incorrect, approach would be to do this on
mini-batches, instead of the entire dataset. Projecting each mini-batch onto the
space of rank $r$ matrices does not guarantee that the activation matrix of the
entire dataset will be of rank $r$, as each of these mini-batches can lie in
very different subspaces. As a simple example, consider the set of coordinate
vectors which can be looked at as rank one matrices corresponding to activations
in batches of size one. However, when these coordinate vectors are stacked
together to form a matrix they create the identity matrix, which is a full rank
matrix.

 
Computational issues aside, another crucial problem stems
from the fact that the activation matrix $\vec{A}_\ell = f^{-}_\ell(.;
\phi)$  is itself parameterised by $\phi$ and thus $\phi$ needs to be
updated in a way such that the generated $\vec{A}_\ell$ is low
rank. It is not immediately clear how to use the low-rank projection
of $\vec{A}_\ell$ to achieve this.
One might suggest to first fully train the network and then obtain low-rank
projections of the activations. Our experiments show that this procedure does
not provide the two main benefits we are looking for: preserving accuracy under
compression and robustness. 














\paragraph{Low-Rank regulariser:} We now describe our regulariser that
encourages learning low-rank activations, and, if optimised properly, guarantees that the rank of the activation matrix (of any
size) will be  bounded by $r$. %
The primary ingredient of our approach is the introduction of an auxiliary
parameter~$\vec{W}\in\reals^{m\times m}$ in a way that allows us to 
shift the low-rank constraint from the activation
matrix $\vec{A}_\ell$~(as in~\Cref{eq:opt_prob}) to 
$\vec{W}$ providing the following two advantages: The rank constraint is now 

\begin{enumerate}
  \item  on a matrix that is independent
of the batch/dataset size, and
\item  on a parameter as opposed to a
data-dependent intermediate tensor~(like activations), and can thus be updated
directly at each iteration. 
\end{enumerate}
Combining these ideas, our final augmented objective function, with the
regulariser, is:
\begin{align}
  \label{eq:aug_opt_2}
  &\min_{\theta, \phi, \vec{W}, \vb} \mathcal{L}(\vec{X}, \vec{Y}; \theta, \phi) + \lambda_1\mathcal{L}_c(\vec{A}_\ell; \vec{W},\vb) + \lambda_2\mathcal{L}_n(\vec{A}_\ell) \\
  &\text{s.t.,} \vec{W}\in \mathbb{R}^{m\times m}, \rank{\vec{W}} = r,~ \vb\in \mathbb{R}^m,\vec{A}_\ell=f^{-}_\ell(\vec{X}; \phi),\nonumber
\end{align}
where,
\begin{align}
  \label{eq:aug_opt_3}
  \mathcal{L}_c(\vec{A}_\ell; \vec{W}, \vb) = \frac{1}{n}\sum_{i=1}^{n}\norm{\vec{W}^\top(\va_i+\vb) - (\va_i+\vb)}_2^2, 
   &\text{and} \; \; \mathcal{L}_n(\vec{A}_\ell) = \frac{1}{n}\sum_{i=1}^n \Big|1 - \norm{\va_i}\Big|.\nonumber
\end{align}
 

 
\noindent Here, $\mathcal{L}_c$ is the projection loss that
ensures that the affine low-rank mappings~($\vec{A}\vec{W}$) of the activations
are close to the original ones i.e. $\vec{AW} \approx \vec{A}$. As the constraint \((\rank{\vec{W}} = r)\) ensures that $\vec{W}$ is
low-rank, $\vec{A}\vec{W}$ is also low-rank and thus implicitly~(due to
$\vec{A}\vec{W}\approx\vec{A}$), $\mathcal{L}_c$ forces the original activations $\vec{A}$ to
be low-rank. The bias $\vb$ allows for the activations to be translated before
projection.%
\footnote{We use the term \emph{projection} loosely as we do not strictly
constrain $\vec{W}$ to be a projection matrix.}

However, note that setting $\vec{A}$ and $\vb$ close to zero trivially minimises
$\mathcal{L}_c$, especially when the activation dimension is large. Also, due to
the positive homogeneity of each layer, the magnitude of the activations can be
minimised in a layer by multiplying the weights of that layer by a small
constant $c$ and then maximised in the next layer by multiplying the weights of
that layer with $\frac{1}{c}$ thereby preserving the final logit magnitudes. We
observed this to happen in practice as it is easier for the network to learn
$\phi$ such that the activations and the bias are very small to
minimise $\mathcal{L}_c$ as compared to learning a low-rank representation space. To prevent this, we use $\mathcal{L}_n$ that acts as a
norm constraint on the activation vector to keep the activations sufficiently
large. Lastly, as the rank constraint is now over $\vec{W}$ and $\vec{W}$ is a
{\em global} parameter independent of the dimension~$n$~(i.e. size of
mini-batch/dataset), we can use mini-batches to optimise~\Cref{eq:aug_opt_2}.
Since $\rank{\vec{AW}} \leq r$ for any $\vec{A}$, optimizing over mini-batches
still ensures that the entire activation matrix is low-rank. Intuitively, this
is because the basis vectors of the low-rank affine subspace are
now captured by the low-rank parameter $\vec{W}$. Thus, as long as $\cL_c$ is
minimised for all mini-batches, $\vec{A} \approx \vec{A}\vec{W}$ holds for
the entire dataset, leading to the low-dimensional support. Thus, the overall
goal of the augmented objective function in~\Cref{eq:aug_opt_2}, is to jointly
penalise the activations~($\vec{A}_\ell$) to make them low-rank and learn the
corresponding low-rank identity map~$\br{\vec{W},b}$. Note, implementation wise,
our regulariser requires adding a  virtual (does not modify the main network)
branch with parameters $\br{\vec{W},b}$ at layer $\ell$. This branch is removed
at the time of inference as the activations learned, by virtue of our objective
function, are already low-rank.

\begin{remark}
  The reason we need to minimise both the reconstruction loss $\cL_c$ and the
  norm constraint loss $\cL_n$ simultaneously is the same as why the spectral
  norm and the stable rank can be independently minimised in
  ~\Cref{chap:stable_rank_main} without affecting each other. To see why, note
  that the rank and the stable rank of the matrix is independent of the scale of
  the matrix i.e. the matrix can be multiplied by any non-zero scalar without
  affecting the rank or the stable rank of the matrix whereas multiplying the
  matrix by a scalar affects the spectral norm proportionally.
\end{remark}

  
\paragraph{Hyper-parameters}
While our algorithm has three hyper-parameters $\lambda_1,\lambda_2$ and $r$, in
  practice, our approach is insensitive to $\lambda_1,\lambda_2$ and thus, we
  set $\lambda_1=\lambda_2=1$. This is an added advantage given the resources
  needed to do hyper-parameter optimisation. In the classical view of
  regularisation e.g. ridge regression, the regularisation coefficient induces a
  bias-variance trade-off i.e. as $\norm{W}_{\mathrm{F}}\rightarrow 0$, the
  accuracy decreases. In our case, under the assumption that there exist
  low-rank representations achieving zero classification error, even as the
  terms $\cL_n$ and $\cL_c$ go to 0, the original classification loss $\cL$ does
  not (necessarily) increase. One way of thinking about this is that the terms
  $\cL_n$ and $\cL_c$ are guiding the optimisation to specific minimisers of the
  empirical classification loss, of which there will necessarily be several
  because of overparameterisation. To verify this empirically, we ran
  experiments with all combinations of $\lambda_1,\lambda_2$ chosen from
  $\bc{1., 0.1, 0.01}$. We observe that for all these settings, the terms
  $\cL_n$ and $\cL_c$ go to 0 while the original loss does not degrade at all.
\begin{algorithm}[t]  \centering
  \caption{Low-Rank (LR) regulariser}
  \label{alg:lr_layer_main}
  \begin{algorithmic}
  \INPUT Activation Matrix $\vec{A}_l$, gradient input ${\bf g}_l$
  \STATE ${\bf Z} \gets (\vec{A}_l+\vb)^\top \vec{W}$
    \COMMENT {forward propagation towards
      the virtual LR layer}
    \STATE $\mathcal{L}_c \gets \frac{1}{b} \norm{{\bf Z} - (\vec{A}_l +
        \vb)}_2^2$ \COMMENT{the reconstruction loss} 
    \STATE $\mathcal{L}_n \gets
      \frac{1}{b}\sum_{i=1}^{b}\big\vert\mathbf{1} - \norm{\va_i}
      \big\vert$ \COMMENT{norm constraint loss}
    \STATE ${\bf g}_W \gets \frac{\partial \mathcal{L}_c}{\partial
        \vec{W}},\enskip {\bf g}\gets {\bf g}_l +
      \frac{1}{b}\sum_{i=1}^{b}\frac{\partial (\mathcal{L}_c +
        \mathcal{L}_n)}{\partial \va_i}$
    \STATE $\vec{W} \gets \vec{W} - \lambda {\bf
        g}_W$ %
    \STATE $\vec{W} \gets
      \prnk{k}{\vec{W}}$ \label{alg:hard_thresh_step} \COMMENT{hard
      thresholds the rank of $\vec{W}$} 
    \OUTPUT ${\bf g}$
    \COMMENT{the gradient to be passed to the layer before}
  \end{algorithmic}
\end{algorithm} 



   
\begin{figure}[t]\centering
  \scalebox{0.49}{\begin{tikzpicture} \node [tensors] (data) {
        \Large$\mathbf{X}$}; \node [tensors, above=3cm of data]
      (activations) { \large$\mathbf{A}$}; \node [rectangle,
      rounded corners, above right=0.8cm of data, yshift=-0.4cm,
      xshift=-0.5cm] (fwd_lbl) { \Large Forward Pass}; \node
      [tensors, above=2.5cm of activations] (output) {
        \large$\mathcal{L}$}; \node [temp_tensors, above right
      =3.5cm of activations, yshift=-1cm] (recons) {
        \large$\mathcal{L}_c$}; \node [temp_tensors, above left
      =3.5cm of activations, yshift=-1cm] (normed) {
        \large$\mathcal{L}_n$};
      % % Draw the links between forces
      \draw[->, thick, color=black, line width=1pt] ([xshift=1 *
      0.1 cm]data.north)-- node[midway, parameters]
      {\normalsize$f_{\ell}^{-}(\mathbf{X};\phi)$} ([xshift=1 *
      0.1 cm]activations.south); \draw[->, dotted, color=black,
      line width=1pt] ([xshift=-1 * 0.1 cm]data.north)--
      ([xshift=-1 * 0.1 cm]activations.south);

      \draw[->, thick, color=black, line width=1pt] ([xshift=1 *
      0.1 cm]activations.north) -- node[parameters, align=center,
      midway] {\normalsize$f_{\ell}^{+}(\mathbf{X};\theta)$}
      ([xshift=1 * 0.1 cm]output.south); \draw[->, dotted,
      color=black, line width=1pt] ([xshift=-1 * 0.1
      cm]activations.north) -- ([xshift=-1 * 0.1 cm]output.south);

      \draw[->, thick, color=black, line width=1pt] (activations)
      -- node[parameters, midway,above, sloped]
      {\normalsize$\mathbf{W},\mathbf{b}$} (recons); \draw[->,
      thick, color=black, line width=1pt] (activations) --
      (normed);
    \end{tikzpicture}}\hspace{15pt}
  \scalebox{0.49}{\begin{tikzpicture} \node [tensors] (data) {
        \Large$\mathbf{X}$}; \node [tensors, above=3cm of data]
      (activations) { \Large$\mathbf{A}$}; \node [tensors,
      above=2.5cm of activations] (output) { \Large$\mathcal{L}$};
      \node [temp_tensors, above right=3.5cm of activations,
      yshift=-1cm] (recons) { \Large$\mathcal{L}_c$}; \node
      [temp_tensors, above left=3.5cm of activations, yshift=-1cm]
      (normed) { \Large$\mathcal{L}_n$}; \node [ rounded corners,
      dashed, above right=0.8cm of data, xshift=-0.5cm,
      yshift=-0.4cm] (fwd_lbl) {\Large Backward
        Pass};% % Draw the links between forces
      \draw[->, thick, color=black, line width=1pt] ([yshift=0 *
      0.1 cm]activations.south) -- node[midway, parameters, below,
      sloped, rotate=180]
      {$\mathbf{g} =\mathbf{g}_c + \mathbf{g}_\ell +\mathbf{g}
        _n$} node[parameters, above, sloped,
      rotate=180]{$\phi=\phi-\eta\frac{\partial
          \mathcal{A}}{\partial \phi}\cdot \mathbf{g}$} ([yshift=0
      * 0.1 cm]data.north);


      \draw[->, thick, color=black, line width=1pt] (output) --
      node[parameters, below, sloped, rotate=180]
      {\normalsize$\mathbf{g}_l=\frac{\partial
          \mathcal{L}}{\partial A}$} node[parameters, above,
      sloped, rotate=180, allow upside
      down]{$\theta=\theta-\eta\frac{\partial
          \mathcal{L}}{\partial \theta}$}(activations) ;


      \draw[->, thick, color=black, line width=1pt] (recons) --
      node[parameters, midway,above, sloped,
      align=center]{$\mathbf{W}=\mathbf{W}-\eta\mathbf{g}_W$ }
      node[parameters, midway,below, sloped, align=center,
      sloped]{\normalsize
        $\mathbf{g}_c = \frac{\partial \mathcal{L}_C}{\partial A}$
      } (activations);


      \draw[->, thick, color=black, line width=1pt] (normed) --
      node[parameters,
      midway,sloped,below,align=center]{\normalsize
        $\mathbf{g}_n = \frac{\partial \mathcal{L}_n}{\partial A}$
      } (activations);

      % \draw[->, dotted, color=black, line width=1pt,
      % yshift=-1cm] ([yshift=-1 * 0.1 cm]activations.west) --
      % node[midway, parameters, below]
      % {\large$\mathbf{g_\ell} + \mathbf{g_C}$} ([yshift=-1 * 0.1
      % cm]data.east); \draw[->, dotted, color=black, line
      % width=1pt] (activations) -- node[parameters, below]
      % {\large$f_{\ell}^{+}(\mathbf{X};\theta)$} (output);
      % \draw[->, dotted, color=black, line width=1pt]
      % (activations) -- node[parameters, midway,below, sloped]
      % {\large$\mathbf{W},\mathbf{b}$} (recons); \draw[->,
      % dotted, color=black, line width=1pt] (activations) --
      % (normed);

    \end{tikzpicture} }
  % \caption{FOSS in Chrome influences industry structure by
  % increasing competition}
  \caption[Illustration of forward and backward propagation of the LR
  Layer]{{\small \bf The LR layer}. The left figure shows the {\em forward
  pass}, {\em solid edges} show the flow of data during training, {\em dashed
  edges}- the flow of data during inference, and {\em dashed nodes} are the {\em
  virtual layer}. The right figure shows the {\em backward pass}.}
  \label{fig:LRtikz}
\end{figure}


\subsection{Algorithm for LR Layer}
\label{sec:alg-lr}

We solve our optimisation problem~(\Cref{eq:aug_opt_2}) by adding a
\emph{virtual} low-rank layer that penalises representations that are far from
their closest low-rank affine representation. Algorithm~\ref{alg:lr_layer_main} %(further details in Appendix~\ref{sec:alg-lr})
describes the operation of the low-rank virtual layer for a mini-batch of size
$b$. We present a flow diagram for the same in Figure~\ref{fig:LRtikz}. This
layer is virtual in the sense that it only includes the parameters $\vec{W}$ and
$\vb$ that are not used  in the NN model itself to make predictions, but
nonetheless, the corresponding loss term $\mathcal{L}_c$ does affect the model
parameters through gradient updates.~\Cref{fig:illus-lr-train} provides an
illustration of how the LR-Layer is added during training as a plug-and-play
layer and then removed during testing, and the generated features are already
low rank. Algorithm~\ref{alg:lr_layer_main} alternately minimises the augmented
loss function in~\Cref{eq:aug_opt_2} and projects the auxiliary parameter
$\vec{W}$ to the space of low-rank matrices. 

% The algorithm is reminiscent of the
% Singular Value Projection~(SVP) Algorithm~\citep{jain2010guaranteed}. However,
% to make the algorithm practical for high dimensional representation spaces, we
% use ensembled Nystr\"om SVD~\citep{williams2001using, halko2011finding,
% kumar2009ensemble} for the projection. We describe the algorithm in
% detail in the next section.


% \begin{algorithm}[h!]  \centering
%    \caption{LR Layer}
%    \label{alg:lr_layer}
%    \begin{algorithmic}[1]
%      \STATE {\bfseries Input:} Activation Matrix $A$, Grad\_input $g$\\
%      \STATE{\bfseries Forward Propagation}
%      \STATE{$Z  \gets W^\top(A+\vb)$}\footnotemark \COMMENT{Compute the affine \textit{Low rank} projection}
%      \STATE {\bfseries Output : $A$}\COMMENT{Output the original activations for the next layer}\\
%      \STATE{\bfseries Backward Propagation} \STATE {$D_1 \gets \frac{\lambda_1}{n} \norm{Z - (A + \vb)}_2^2$}
%      \COMMENT{Computes the reconstruction loss $\mathcal{L}_c$}
%      \STATE {$D_2\gets \frac{\lambda_2}{n}\sum_{i=0}^{n-1}\big\vert\mathbf{1} - \norm{\va_i} \big\vert$}
%      \COMMENT{Computes the loss for the norm constraint $\mathcal{L}_N$}
%      \STATE {$D\gets D_1 + D_2$}
%      \STATE {$g_W \gets \frac{\partial D}{\partial W}, g_i\gets g + \frac{1}{n}\sum_{i=0}^{n-1}\frac{\partial D}{\partial \va_i}$}
%      \STATE{\bfseries Output : $g_i$}
%      \COMMENT{Outputs the gradient to be passed to the layer before}\\
%      \STATE{\bfseries Update Step}
%      \STATE{$W \gets W - \lambda g_W$}\COMMENT{Updates the weight with the gradient from $D$.}\\
%      \STATE{$W\gets \prnk{k}{W}$ \label{alg:hard_thresh_step}}\COMMENT{Hard thresholds the rank of $W$}
% \end{algorithmic}
% \end{algorithm} \footnotetext{$\vb + A$ is computed by adding $\vb$ to
% every row in $A$}

\begin{figure}
  \centering
  \begin{subfigure}[c]{0.65\linewidth}
    \includegraphics[width=0.99\linewidth]{./low_rank_folder/figs/lr_training.png}
    \caption{Training}
    \label{fig:illus-train}
  \end{subfigure}\vspace{10pt}
  \begin{subfigure}[c]{0.65\linewidth}
  \includegraphics[width=0.99\linewidth]{./low_rank_folder/figs/lr_inference.png}
  \caption{Testing}
  \label{fig:illus-test}
  \end{subfigure}
  \caption{\Cref{fig:illus-train} shows an illustration of how the LR-Layer is added as a plug-and-play layer during training.~\Cref{fig:illus-test} shows an illustration that the LR layer is removed during testing and the generated representations are already low-rank.}
  \label{fig:illus-lr-train}
\end{figure}

The rank projection step in~\Cref{alg:lr_layer_main} is executed by a hard
thresholding operator $\prnk{r}{W}$, which finds the best $r$-rank approximation
of $W$. Essentially, $\prnk{r}{W}$ solves the following optimisation problem,
which can be solved using singular value decomposition (SVD).

\begin{equation}
  \prnk{r}{W} = \argmin_{\rank{Z} = r}\norm{W
                                - Z}_F^2 
 \end{equation}

 However, the projection can be very expensive due to the large dimension of the
representations space~(e.g. $16000$). To get around this, we use the ensembled
Nystr\"om SVD algorithm~\citep{williams2001using, halko2011finding,
kumar2009ensemble}.
%
  
    
\paragraph{Handling large activation
matrices}: %\label{sec:handl-large-activ}
%
Singular Value Projection~(SVP) introduced in ~\citet{jain2010guaranteed} is an
algorithm for rank minimisation under affine constraints. In each iteration, the
algorithm performs gradient descent on the affine constraints alternated with a
rank-k projection of the parameters and it provides recovery guarantees under
weak isometry conditions. However, the algorithm has a complexity of $O(mnr)$
where $m, n$ are the dimensions of the matrix and $r$ is the desired low rank.
Faster methods for SVD of sparse matrices are not applicable as the matrices in
our case are not necessarily sparse.  We use the ensembled Nystr\"om
method~\citep{williams2001using, halko2011finding, kumar2009ensemble} to boost
our computational speed at the cost of the accuracy of the low-rank
approximation. It is essentially a sampling-based low-rank approximation to a
matrix. The algorithm is described in detail in~\Cref{sec:ensembl-nystr-meth}.
Though the overall complexity for projecting $W$ remains $O(m^2r)$, the
complexity of the hard-to-parallelise SVD step is now $O(r^3)$, while the rest
is due to matrix multiplication, which is fast on modern GPUs.

The theoretical guarantees of the Nystr\"om method hold only when the weight
matrix of the \lr is symmetric and positive semi-definite (SPSD) before each
$\prnk{r}{\cdot}$ operation. Note that the PSD constraint is actually not a
restriction as all projection matrices are PSD by definition.  For example, on
the subspace spanned by columns of a matrix $\vec{X}$, the projection matrix is
$\vec{P} = \vec{X}(\vec{X}^\top \vec{X})^{-1}\vec{X}^\top$, which is always PSD.
We know that a symmetric diagonally dominant real matrix with non-negative
diagonal entries is PSD. With this motivation, the matrix $\vec{W}$ is
smoothened by repeatedly adding $0.01\vec{I}$ until the \textsf{SVD} algorithm
converges where $\vec{I}$ is the identity matrix.\footnote{The computation of
the singular value decomposition sometimes fail to converge if the matrix is
ill-conditioned}. This is a heuristic to make the matrix well-conditioned as
well as diagonally dominant and it helps in the convergence of the algorithm
empirically. 

\paragraph{Symmetric Low-Rank Layer}%\label{sec:symmetric-low-rank}

The symmetricity constraint restricts the projections allowed in our
optimisation, but empirically this restriction does not seem to hurt its
performance. Implementation wise, gradient updates may make the matrix parameter
asymmetric, even if we start with a symmetric matrix. Reparameterising the \lr
fixes this issue; the layer is parameterised using $\vec{W}_s$ (to which
gradient updates are applied), but the layer projects using $\vec{W} =
(\vec{W}_s + \vec{W}_s^\top)/2$, which is by definition a symmetric matrix.
After the rank projection is applied to the (smoothed version of) $\vec{W}$,
$\vec{W}_s$ is set to be $\prnk{r}{\vec{W}}$. By~\Cref{thm:nystrom_sym}, if we
start with an SPSD matrix $\vec{W}_s$, the updated $\vec{W}_s$ is an SPSD
matrix. As a result, the updated $\vec{W}$ is also SPSD.

\begin{restatable}[Column Sampled Nystr\"om approximation preserves SPSD matrices]{lem}{spsdnystrom}
  \label{thm:nystrom_sym} If $\vec{X}\in\reals^{m\times m}$ is an SPSD matrix
and $\vec{X}_r\in\reals^{m\times m}$ is the best Nystr\"om ensembled, column
sampled r-rank approximation of $\vec{X}$, then $\vec{X}_r$ is SPSD as
well.

Proof in~\Cref{sec:lr-spsd-proof}
\end{restatable}


\subsection{Ensembled Nystr\"om method}
\label{sec:ensembl-nystr-meth}


 Let $\vec{W}\in \reals^{m\times m}$ be a symmetric positive semidefinite matrix
(SPSD). We want to generate a matrix $\vec{W}_r$ which is an r-rank approximation
of $\vec{W}$ without performing SVD on the full matrix $\vec{W}$ but only on a
principal submatrix of $\vec{W}$. A principal submatrix of a matrix $\vec{W}$ is
a square matrix formed by removing some columns and the corresponding rows from
$\vec{W}$~\citep{Meyer2000MAA}. Let the principal submatrix be $\vec{Z}\in
\reals^{l\times l}$, where $l\ll m$. We construct $\vec{Z}$ by first sampling
$l$ indices from the set $\{1\ldots m\}$ and selecting the corresponding columns
from $\vec{W}$ to form a matrix $\vec{C}\in \reals^{m\times l}$. Then, we select
the $l$ rows with the same indices from $\vec{C}$ to get $\vec{Z}\in
\mathbb{R}^{l \times l}$. We can rearrange the columns of $\vec{W}$ and
$\vec{C}$ so that \[W =
\begin{bmatrix} \vec{Z} \quad \vec{W}_{21}^T \\
  \vec{W}_{21}\quad \vec{W}_{22} \end{bmatrix} \quad \quad \vec{C} =
  \begin{bmatrix} \vec{Z} \\ \vec{W}_{21}
  \end{bmatrix}
\] According to the Nystr\"om approximation, the low-rank
approximation of $\vec{W}$ can be written as
\begin{equation}
  \label{eq:nystrom_approx} \vec{W}_r = \vec{C} \vec{Z}_r^{+}\vec{C}^T
\end{equation} where $\vec{Z}_r^{+}$ is the pseudo-inverse of the best $r$
rank approximation of $\vec{Z}$. Hence, the entire algorithm is as follows.
\begin{itemize}
\item Compute $\vec{C}$ and $\vec{Z}$ as stated above.
\item Compute the top $r$ singular vectors and values of $\vec{Z}$ : $\vec{U}_r,~\mathbf{\Sigma}_r,~\vec{V}_r$.
\item Invert each element of $\mathbf{\Sigma}_r$ to get the Moore pseudo-inverse of
$\vec{Z}_r$.
\item Compute $\vec{Z}_r^{+} = \vec{U}_r\mathbf{\Sigma}_r^{-1} \vec{V}_r$ and $\vec{W}_r = \vec{C}
\vec{Z}_r^{+}\vec{C}^T$.
\end{itemize} Though by trivial computation, the complexity of the
algorithm seems to be $O(l^2r + ml^2 + m^2l) = O(m^2r)$~(in our
experiments $l = 2r$), however the complexity of the SVD
step is only $O(r^3)$ which is much lesser than $O(m^2r)$ and while
matrix multiplication is easily parallelisable, SVD is not.

To improve the accuracy of the approximation, we use the ensembled Nystr\"om
sampling-based methods~\citep{kumar2009ensemble} by averaging the outputs of $t$
runs of the Nystr\"om method. The $l$ indices for selecting columns and rows are
sampled from a uniform distribution and it has been
shown~\citep{kumar2009sampling} that uniform sampling performs better than most
other sampling methods. Theorem 3 in ~\citet{kumar2009ensemble} provides a
probabilistic bound on the Frobenius norm of the difference between the exact
best r-rank approximation of $\vec{W}$ and the Nystr\"om sampled r-rank
approximation.


==> sparsity.tex <==

A criterion for reducing redundancy, which has been fairly well studied in literature, in DNNs is to promote sparsity in the parameter space (as mentioned above). While the problem of optimisation under $\ell_0$ constraints has been well studied for linear models, it is still a challenge in deep models. There are two main problems in promoting sparsity in neural networks - along with devising the right optimisation algorithm for enforcing the $\ell_0$ constraints one has to account for how these imposed constraints interact with the special structures (eg. convolutional filters) and restrictions (eg. weight tying)  that are already present in the structure of various kinds of networks eg. CNNs and RNNs. The second problem, which  is more practical, is to promote the sparsity in a way so as to be able to reap maximum benefit in terms of computational efficiency and/or in performance.  As we will see below, in a few such works that I have studied this term, the problem is more well studied for CNNs than it is with RNNs and different papers focuses on different aspects of it. 

The filters in CNN map a certain section of the input to a higher order feature (eg. lines, arcs, faces etc). ~\citet{wen2016learning} considers the problem of reducing the number of filters  i.e., by treating each CNN filter as one unit, group sparsity is promoted in convolutional neural networks with a group LASSO kind of regularization. Another benefit of using group lasso is that one doesn't need to specify the sparsity hyper-parameter, which one would have needed to if something akin to group $\ell_0$ regularization was used.  For a CNN, they define the loss function as
    \begin{equation}
      \label{eq:1}
      E(W) = E_D(W) + \lambda_n \sum_{l=1}^L(\sum_{n_l=1}^{N_l} \|W_{n_l,:,:,:}^{(l)}\|_g) + \lambda_c\cdot \sum_{l=1}^L(\sum_{c_l=1}^{C_l} \|W_{:,c_l,:,:}^{(l)}\|_g)
    \end{equation}
    where $W^{(l)} \in \mathbb{R}^{N_l\times C_l\times M_l \times K_l}$. Intuitively, this regards a convolutional filter as a unit instead of regarding a pixel as a unit. %
    They also look at some other groups of units like entire layers. The implementation is not, however, straightforward and has a few quirks. \footnote{Please read section 4.2 in ~\citet{wen2016learning}.}
    It is to be noted that their  motivation for promoting sparsity is to get a compressed network for computational reasons and to not look at it as a regularization to help performance as, though it results in speedups, gains in performance is not observed.


    Where ~\citet{wen2016learning} looks at the structure of the parameters of a CNN, it doesn't take into account the behaviour of the convolution operator. An important property of the convolution operator is that it employs a huge amount of weight tying by using the same set of weights to do similar operations simultaneously on different parts of the input. This, though makes it highly parallelizable, makes it very expensive  were it to run on a single thread. ~\citet{liu2015sparse} increases the speed of the convolution operator faster by constructing low rank sparse approximations of the convolution kernel. Computationally this approximation reduces a convolution operator to a multiplication of two sparse matrices. I give a rough description of the main idea in the appendix. \footnote{The detailed algorithm is listed in \textbf{Section 3.1} in ~\cite{liu2015sparse}.}\\
    
    Most of the results  reported in the paper is on the theoretical  and the actual speedup obtained by their networks. They work with a model similar to Alexnet on the ILSVRC12 and obtain a speedup of atleast $2.47\% $ (on the first convolution layer) and a maximum of  $6.88\%$ (on the the third layer). On the task of  object detection(PASCAL VOC2007), SPP net and obtains a speedup of around $7x$ while suffering an accuracy drop of $2\%$


    Neither \citet{wen2016learning} nor \cite{liu2015sparse} enforces sparsity directly on their models. The only two papers~\citep{han2016dsd, Jin2016}, that I have found to do so, use the iterative hard thresholding( IHT) method~\citep{blumensath2009iterative}, a method for performing direct $\ell_0$ regularization. %

    The first step in their algorithms is sparsifying a neural network by performing on each layer a hard thresholding operation to achieve a desired (pre-fixed) level of layer wise sparsity. The second step is to perform a fully corrective step, for $s_1$ epochs, through gradient descent on the supports that remain.

    Once a fine-tuned sparse network is achieved, they loosen the sparsity  assumption to include the rest of the weights (zero initialized) and perform another fully corrective step, for $s_2$ epochs, through gradient descent on the entire network. Therefore, it alternates between sparse and dense training. Where~\citet{han2016dsd} creates a dense network by doing this sequence dense-sparse-dense training only once,~\citet{Jin2016} repeats the steps over and over again to obtain (though they don't mention sparsifying at the end) a final sparse network. %


Though not promoting sparsity,~\citet{HMD:2016} provides a very aggressive network compression technique. Look in the appendix for a more detailed description of the technique.



==> stable_rank_folder/__latexindent_temp.tex <==
\section{Experiments on a discriminative setup}
\label{sec:experiments-srn}
\paragraph{Dataset and architectures} For classification, we perform experiments
on ResNet-110~\citep{HZRS:2016}, WideResNet-28-10~\citep{Zagoruyko2016},
DenseNet-100~\citep{Huang2017}, VGG-19~\citep{simonyan2014very}, and
AlexNet~\citep{krizhevsky2009learning} using the CIFAR100 and
CIFAR10~\citep{krizhevsky2009learning} datasets. We train them using standard
training recipes with SGD, using a learning rate of $0.1$~(except AlexNet where
we use a learning rate of $0.01$), and a momentum of $0.9$ with a batch size of
$128$ (further details in Appendix~\ref{sec:expr-settings}). In addition to
training for a fixed number of epochs, we also present results where the
training accuracy~(as opposed to the number of iterations) is used as a stopping
criterion to show that our regulariser performs well with a range of stopping
criteria.

For GAN experiments, we use CIFAR100, CIFAR10, and
CelebA~\citep{liu2015faceattributes} datasets. We show results on both,
conditional and unconditional GANs. Please refer to~\cref{sec:expr-settings} for
further details about the training setup.

\paragraph{Choosing stable rank} Given a matrix $\vec{W} \in \reals^{m \times
  n}$, the desired stable rank $r$ is controlled using a single
hyperparameter $c$ as $r = c \; \min(m,n)$, where $c \in (0, 1]$.
For simplicity, we use the same $c$ for all the linear layers. 
Note that if $c=1$, or for a given $c$, if $\srank{\vec{W}} \leq r$,
then SRN boils down to SN. For classification, we choose $c = \{0.3, 0.5\}$, and compare SRN against standard
training (Vanilla) and training with \gls{sn}. For GAN experiments, we choose $c = \{0.1, 0.3, 0.5, 0.7, 0.9\}$, and
compare SRN-GAN against SN-GAN~\citep{miyato2018spectral}, WGAN-GP~\citep{Gulrajani2017}, and orthonormal regularisation GAN
(Ortho-GAN)~\citep{Brock2016}.



\begin{figure}[t]
  \centering\small
  \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/r110_test.pdf_tex}
    \subcaption{ ResNet110}
  \end{subfigure}
  \begin{subfigure}[!t]{0.21\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/wrn_test.pdf_tex}
    \subcaption{ WideResNet28}
  \end{subfigure}
   \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/alex_test.pdf_tex}
    \subcaption{ Alexnet}
  \end{subfigure}
  \begin{subfigure}[!t]{0.19\linewidth}
    \def\svgwidth{0.99\linewidth}
    \input{./stable_rank_folder/figs/dens_test.pdf_tex}
    \subcaption{ Densenet-100}
  \end{subfigure}
   \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/vgg_test.pdf_tex}
    \subcaption{ VGG-19}
  \end{subfigure}
  \caption[Test accuracies on CIFAR100 with fixed number of training epochs]{Test accuracies on CIFAR100 for clean data using the number of epochs as stopping criterion. Higher is better.}
  \label{fig:test-acc}
\end{figure}

\begin{figure}[t]
  \centering\small
  \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/c10_r110_test.pdf_tex}
    \subcaption{ResNet110}
  \end{subfigure}
  \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/c10_wrn_test.pdf_tex}
    \subcaption{WideResNet28}
  \end{subfigure}
   \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/c10_alex_test.pdf_tex}
    \subcaption{ Alexnet}
  \end{subfigure}
  \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/c10_dens_test.pdf_tex}
    \subcaption{ Densenet-100}
  \end{subfigure}
  \caption[Test error on CIFAR10 with fixed number of training epochs]{Test accuracies on CIFAR10 for clean data using the number of epochs as stopping criterion. Higher is better.}
  \label{fig:test-acc-epoch-c10}
\end{figure}

\subsection{Classification experiments}\label{sec:gen_exp_results} We perform
each experiment $5$ times using a new random seed each time and report the mean and the $75\%$ confidence interval for the test error. We plot the test accuracy
on CIFAR100 in~\cref{fig:test-acc} and CIFAR10
in~\cref{fig:test-acc-epoch-c10}.

These experiments show that the test accuracy of \gls{srn} on a wide variety
\gls{nn}s is always higher than the Vanilla and SN (except for SRN-50  on
Alexnet where \gls{srn} and \gls{sn} are almost equal). However, \gls{sn}
performs slightly worse than Vanilla for WideResNet-28 and ResNet110. The fact
that \gls{srn} also involves \gls{sn}, combined with the above observation,
indicates that even though \gls{sn} reduced the learning capability of these
networks, normalizing stable rank must have improved it significantly in order
for \gls{srn} to outperform Vanilla. For example, in the case of ResNet110,
\gls{sn} is $71.5\%$ accurate whereas \gls{srn} provides an accuracy of
$73.2\%$. In addition to this, we also note that even though \gls{sn} is used
extensively for the training of GANs, it is not a popular choice when it comes
to training standard \gls{nn}s for classification. We suspect that this is
because of the decrease in performance, we observe here. Hence, as our
experiments indicate that~\Gls{srn} overcomes this,~\Gls{srn} could be a
potentially important regulariser in the classification setting.

\begin{figure}
  \centering\small
  \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/r110_rand.pdf_tex}
    \subcaption{ResNet110}
  \end{subfigure}
     \begin{subfigure}[!t]{0.21\linewidth}
    \def\svgwidth{0.99\linewidth}
    \input{./stable_rank_folder/figs/wrn_rand.pdf_tex}
    \subcaption{WideResNet28}
  \end{subfigure}
   \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/alex_rand.pdf_tex}
    \subcaption{Alexnet}
  \end{subfigure}
   \begin{subfigure}[!t]{0.19\linewidth}
    \def\svgwidth{0.99\linewidth}
    \input{./stable_rank_folder/figs/dens_rand.pdf_tex}
    \subcaption{Densenet-100}
  \end{subfigure}
   \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/vgg_rand.pdf_tex}
    \subcaption{VGG-19}
  \end{subfigure}
  \caption[Shattering Experiments on CIFAR100]{Train accuracies on CIFAR100 for shattering experiment. Lower indicates less memorisation, thus, better.}
  \label{fig:rand-acc}
\end{figure}
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.33\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/c10_r110_rand.pdf_tex}
    \caption{ResNet110}\label{fig:r100-rand-train-c10}
  \end{subfigure}
  \begin{subfigure}[t]{0.33\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/c10_alex_rand.pdf_tex}
    \caption{Alexnet}\label{fig:alex-rand-train-c10}
  \end{subfigure}
  \caption[Shattering experiments on CIFAR10]{Train accuracies on CIFAR10 for shattering experiment. Lower indicates less memorisation, thus, better.}
  \label{fig:cifar-10-gen}
\end{figure}

\subsection{Shattering experiments}
Our previous set of experiments established that \gls{srn} provides improved
classification accuracies on various \gls{nn}s. Here we study the generalisation
behaviour of these models. Quantifying generalisation behaviour is non-trivial
and there is no clear answer to it. However, we utilise recent efforts that
explore the theoretical understanding of generalisation to study generalisation
of SRN in practice.


To inspect the generalisation behaviour in \gls{nn}s we begin with the
shattering experiment~\citep{Zhang2016}. It is a test of whether the network can
fit the training data well but not a label-randomised version of it (each image
of the dataset is assigned a random label). As $P\bs{y\vert \vec{x}}$ is
essentially uninformative because it is a uniformly random distribution, there
is no correlation between the labels and the data points. Thus, the best
possible test accuracy on this task~(the test labels would also be randomised)
is approximately $1\%$ on CIFAR100~(\(10\%\) in CIFAR10). A high training
accuracy --- which indicates a high generalisation gap (difference between train
and test accuracy) can be achieved only by memorising the train data. In these
experiments, the training of all models of one architecture are stopped after
the same number of epochs, which is double the number of epochs the model is
trained for on the clean datasets. ~\cref{fig:rand-acc} shows that \gls{srn}
reduces memorisation on random labels~(thus, reduces the estimate of the
Rademacher complexity~\citep{Zhang2016}) on CIFAR100.
In~\cref{fig:cifar-10-gen}, we plot the training accuracy on CIFAR10 and observe
a similar result. Importantly, the same model architectures and training
strategy were able to achieve high test accuracy for the clean dataset in the
previous section.
 


\subsection*{Training accuracy as stopping criterion}

We used the number of training epochs as our stopping criterion in the previous
experiments. To show that the results hold consistently across different
stopping criteria, we use a different stopping criterion here. In particular, we
use the training accuracy as a stopping criterion here. For ResNet110,
WideResNet-28, Densenet-100, and VGG-19 we use a training accuracy of $99\%$ as
a stopping criterion and report the test accuracy when that training accuracy is
achieved for the first time. For Alexnet, as SRN-30 never achieves a training
accuracy higher than $55\%$, we use $55\%$ as the stopping criterion and plot
the test accuracies in~\cref{fig:test-acc-stop} for CIFAR100. Our results show
that SRN-30 and SRN-50 outperform SN and vanilla consistently. In
Figure~\ref{fig:test-acc-stop-c10}, we show similar results for CIFAR10. As
AlexNet can achieve higher accuracy for CIFAR10, we use $85\%$ as the
stopping criterion for AlexNet on CIFAR10. 


\begin{figure}[t]
  \centering\small
  \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.99\linewidth}
    \input{./stable_rank_folder/figs/r110_gen_stop.pdf_tex}
    \subcaption{ResNet110}
  \end{subfigure}
  \begin{subfigure}[!t]{0.21\linewidth}
    \def\svgwidth{0.99\linewidth}
    \input{./stable_rank_folder/figs/wrn_gen_stop.pdf_tex}
    \subcaption{WideResNet28}
  \end{subfigure}
   \begin{subfigure}[!t]{0.185\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/alex_gen_stop.pdf_tex}
    \subcaption{Alexnet}
  \end{subfigure}
  \begin{subfigure}[!t]{0.19\linewidth}
    \def\svgwidth{0.99\linewidth}
    \input{./stable_rank_folder/figs/dens_gen_stop.pdf_tex}
    \subcaption{Densenet-100}
  \end{subfigure}
   \begin{subfigure}[!t]{0.19\linewidth}
    \def\svgwidth{0.99\linewidth}
    \input{./stable_rank_folder/figs/vgg_gen_stop.pdf_tex}
    \subcaption{ VGG-19}
  \end{subfigure}
  \caption[Test error on CIFAR100 with early stopping.]{Test accuracies on CIFAR100 for clean data using a stopping
    criterion based on train accuracy. Higher is better.}
  \label{fig:test-acc-stop}
\end{figure}

\begin{figure}[t]
  \centering\small
  \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/r110_c10_gen_stop.pdf_tex}
    \subcaption{ResNet110}
  \end{subfigure}
  \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/wrn_c10_gen_stop.pdf_tex}
    \subcaption{WideResNet-28}
  \end{subfigure}
   \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/alex_c10_gen_stop.pdf_tex}
    \subcaption{ Alexnet}
  \end{subfigure}
  \begin{subfigure}[!t]{0.24\linewidth}
    \def\svgwidth{0.98\linewidth}
    \input{./stable_rank_folder/figs/dens_c10_gen_stop.pdf_tex}
    \subcaption{ Densenet-100}
  \end{subfigure}
  \caption[Test Error on CIFAR10 with early stopping]{Test accuracies on CIFAR10 for clean data using a stopping
    criterion based on train accuracy. Higher is better.}
  \label{fig:test-acc-stop-c10}
\end{figure}

\subsection*{Non-generalisable settings}

So far, we have looked at learning with hyper-parameters like learning rate and
weight decay set to values commonly used in training of deep neural networks.
However, these hyper-parameters have been adjusted through years of practice.
This section looks specifically at  settings that are known to be highly
non-generalisable --- {\em low learning rate and without weight decay}.

First, we look at a WideResNet-28-10 trained with SRN, SN, and vanilla methods
but with a low learning rate of $0.01$ and a small weight decay of $5\times
10^{-4}$ on randomly labelled CIFAR100 for $50$ epochs. The results, shown
in~\cref{tab:low_lr_wrn}, supports our hypothesis that SRN is more robust to
random noise than SN or vanilla methods even in this highly-non generalisable
setup.


\begin{table}[!htb]
  \centering\small
  \begin{tabular}{||c|c|c||}\hline
    Stable-30&Spectral&Vanilla\\\hline
    $\mathbf{29.04}$& $17.24 $ & $1.22$ \\\hline
  \end{tabular}
  \caption[Shattering experiment with low-learning rate]{Training error for WideResNet-28-10 on CIFAR100 with randomised
    labels, low lr$=0.01$, and with weight decay.~(Higher
    is better.)}
  \label{tab:low_lr_wrn}
\end{table}

Secondly, we see whether weight decay provides a further edge to generalisation
when used in combination with SRN and SN. As shown in~\cref{tab:low_lr_rnet},
\gls{srn} consistently achieves lower generalisation error~(by achieving a low
train error) both in the presence and the absence of weight
decay.~\Cref{tab:clean-c100-lowlr} shows it also achieves a higher clean test
accuracy for this setting.  Thus~\Gls{srn} generalises better even with a low
learning rate and is further benefitted by regularisers like weight decay.

\begin{table}[!htb]
  \centering
  \begin{tabular}{l@{\quad}c@{\quad}c@{\quad}c@{\quad}c@{\quad}}\toprule
    &SRN-50&SRN-30&Spectral (SN) &Vanilla\\\midrule
    WD & $\mathbf{12.02 \pm 1.77}$ &$\mathbf{11.87 \pm 0.57}$ & $\mathbf{11.13 \pm 2.56}$ & $\mathbf{10.56
    \pm 2.32}$ \\
    w/o WD & $17.71 \pm 2.30$ &$19.04 \pm 4.53$ & $17.22 \pm 1.94$ & $13.49
    \pm 1.93$ \\\bottomrule
  \end{tabular}
  \caption[Shattering experiment with non-generalisable settings on CIFAR100]{{\bf Highly non-generalisable setting}. Training error
    for ResNet-110 on CIFAR100 with randomised labels, low lr$=0.01$,
    and with and without weight decay.~(Higher is better.)}
  \label{tab:low_lr_rnet}
\end{table}

\begin{table}[!htb]
  \centering
  \begin{tabular}{ccccc}\toprule
    & Vanilla & Spectral & Stable-50 & Stable-30 \\\midrule
    W/o WD & $69.2 \pm 0.5$ & $69\pm 0.1$ & $69.1 \pm 0.85$ & $69.3 \pm 0.4$ \\
    With WD & $\mathbf{70.4 \pm 0.3}$ & $\mathbf{71.35 \pm 0.25}$ & $\mathbf{70.6 \pm 0.1}$ & $\mathbf{70.6 \pm 0.1}$ \\\bottomrule
  \end{tabular}
  \caption[Clean test accuracy  for non-generalisable settings on CIFAR10.]{Clean test accuracy on CIFAR10. The learning configuration
    corresponds to the non-generalisable settings with a high learning
    rate.}
    \label{tab:clean-c100-lowlr}
\end{table}



\subsection{Empirical evaluation of generalisation behaviour}
When all the factors in training~(eg. architecture, dataset, optimiser, among
others) are fixed, and the only variability is in the normalization~(i.e. in SRN
vs SN vs Vanilla), the generalisation error can be written as $
\abs{\mathrm{Train\ Err} - \mathrm{Test\ Err}} \le
\tildeO{\sqrt{\nicefrac{C_{\mathrm{alg}}}{m}}}$ where $\tildeO{\cdot}$ ignores
the logarithmic terms, $m$ is the number of samples in the dataset, and
$C_{\mathrm{alg}}$ denotes a measure of {\em sample complexity} for a given
algorithm i.e. SRN vs SN vs Vanilla. The lower the value of $C_{\mathrm{alg}}$,
the better is the generalisation. This is reminiscent of the basic theorem of
generalisation previously discussed in~\Cref{thm:basic-gen-thm}. In this
section, we measure $C_{\mathrm{alg}}$ as a proxy for measuring generalisation.

First, we restate some of the concepts we had previously discussed
in~\Cref{sec:marg-based-gener-main}. The margin of a network, defined
in~\Cref{defn:margin} at a data point measures the gap in the confidence of the
network between the correct label and the other labels. In the rest of the
section, we will treat $\gamma$ as a random variable depending on the random
variables $\cX$ and $\cY$.
\margin*
We also restate the expressions for $C_{\mathrm{alg}}$ that we used previously in~\Cref{thm:spec-norm-marg-main} and~\Cref{eq:stable-spec-compl}. In addition, we define a new complexity measure from~\citet{wei2019}.

\begin{itemize}
  \item \textbf{Spec-Fro:}
    $\dfrac{\prod_{i=1}^L\norm{\vec{W}_i}_2^2\sum_{i=1}^L\srank{\vec{W}_i}}{\gamma^2}$~\citep{neyshabur2018a}.
    The two quantities used to normalize the margin~($\gamma$) are the product
    of spectral norm i.e. $\prod_{i=1}^L\norm{\vec{W}_i}_2^2$~(or worst case
    lipschitzness) and the sum of stable rank {\em i.e.},
    $\sum_{i=1}^L\srank{\vec{W}_i}$~(or an approximate parameter count like rank
    of a matrix).
  \item \textbf{Spec-L1:} $\dfrac{\prod_{i=1}^L\norm{\vec{W}_i}_2^2
      \br{\sum_{i=1}^L\frac{\norm{\vec{W}_i}_{2,1}^{\nicefrac{2}{3}}}{\norm{\vec{W}_i}_2^{\nicefrac{2}{3}}}}^3}{\gamma^2}$,
  where $\norm{.}_{2,1}$ is the matrix 2-1 norm. As showed
  by~\citet{bartlett2017spectrally}, Spec-L1 is the spectrally
  normalized margin, and unlike just the margin, is a good indicator of the
  generalisation properties of a network. 
  \item \textbf{Jac-Norm:}
    $\sum_{i=1}^L\dfrac{\norm{\vec{h}_i}_2\norm{\vec{J}_i}_2}{\gamma}$~\citep{wei2019},
    where  $\vec{h}_i$ is the $i^{\it th}$ hidden layer and $\vec{J}_i
    =\frac{\partial \gamma}{\partial h_i}$ {\em i.e.}, the Jacobian of the
    margin with respect to the $i^{\it th}$ hidden layer (thus, a vector). Note,
    Jac-Norm depends on the norm of the Jacobian (local empirical \Gls{lip}) and
    the norm of the hidden layers, which are additional data-dependent terms
    compared to Spec-Fro and Spec-L1.
  \end{itemize}
  

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{1.0\linewidth}
    \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\linewidth} \input{./stable_rank_folder/figs/jac_gen_rnet110.pdf_tex}
    \subcaption{R110-Jac-Norm}\label{fig:r110-jac-comp}
  \end{subfigure}\begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\linewidth} \input{./stable_rank_folder/figs/spec_l1_r110.pdf_tex}
    \subcaption{R110-Spec-$L_1$}\label{fig:r110-spec-l1-comp}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\textwidth}
    \input{./stable_rank_folder/figs/spec_fro_r110v1.pdf_tex}
    \subcaption{R110-Spec-Fro}\label{fig:r110-spec-fro-comp}
  \end{subfigure}
\end{subfigure}
\begin{subfigure}[t]{1.0\linewidth}
    \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\linewidth} \input{./stable_rank_folder/figs/jac_gen_wrn.pdf_tex}
    \subcaption{WRN-Jac-Norm}\label{fig:wrn-jac-comp}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\linewidth} \input{./stable_rank_folder/figs/spec_l1_wrn.pdf_tex}
    \subcaption{WRN-Spec-$L_1$}\label{fig:wrn-spec-l1-comp}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\textwidth}
    \input{./stable_rank_folder/figs/spec_fro_wrnv2.pdf_tex}
    \subcaption{WRN-Spec-Fro}\label{fig:wrn-spec-fro-comp}
  \end{subfigure}
\end{subfigure}
\begin{subfigure}[t]{1.0\linewidth}
    \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\linewidth} \input{./stable_rank_folder/figs/jac_gen_dens100.pdf_tex}
    \subcaption{D100-Jac-Norm}\label{fig:d100-jac-comp}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\linewidth} \input{./stable_rank_folder/figs/spec_l1_dens.pdf_tex}
    \subcaption{D100-Spec-$L_1$}\label{fig:d100-spec-l1-comp}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\linewidth}
    \def\svgwidth{0.98\textwidth}
    \input{./stable_rank_folder/figs/spec_fro_dens.pdf_tex}
    \subcaption{D100-Spec-Fro}\label{fig:d100-spec-fro-comp}
  \end{subfigure}
\end{subfigure}
  \caption[Empirical comparison of generalisation bounds]{($\log$) Sample complexity ($C_{\mathrm{alg}}$) of
    ~ResNet-110~(\cref{fig:r110-jac-comp,fig:r110-spec-l1-comp,fig:r110-spec-fro-comp}),
    WideResNet-28-10~(\cref{fig:wrn-jac-comp,fig:wrn-spec-l1-comp,fig:wrn-spec-fro-comp}),
    and Densenet-100~(\cref{fig:d100-jac-comp,fig:d100-spec-l1-comp,fig:d100-spec-fro-comp})
quantified using the three measures discussed in this chapter. Left
is better. Vanilla is omitted
from~\cref{fig:r110-spec-l1-comp,fig:r110-spec-fro-comp,fig:d100-spec-l1-comp,fig:d100-spec-fro-comp}
as it is too far to the right. Also, in situations where SRN-50 and SN performed the same, we removed the histogram to avoid clutter.}
  \label{fig:compl}
\end{figure}

We evaluate the above-mentioned sample complexity measures on $10,000$ points
from the dataset and plot the distribution of its $\log$ using a histogram shown
in~\cref{fig:compl}. The more to the left the histogram is, the smaller is the
value of $C_{\mathrm{alg}}$ and thus the better is the generalisation capacity
of the network.

For better clarity, we report the $90$ percentile mark for each of these
histograms in ~\cref{tab:perc-compl}. As the plots and the table shows, both
\gls{srn} and \gls{sn} produces a much smaller complexity measure than a vanilla
network and in 7 out of the 9 cases, SRN is better than SN. The difference
between SRN and SN is much more significant in the case of Jac-Norm. As the
Jac-Norm depends on the empirical lipschitzness, it provides the empirical
validation of our arguments in~\Cref{sec:stable_rank_alg}.
%Additional details about these experiments are in~\cref{sec:values-compl}.
\begin{table}[!htb]\footnotesize
  \centering\renewcommand{\arraystretch}{1.1}
  \begin{tabular}[t]{C{3cm}C{3cm}c@{\quad}c@{\quad}c@{\quad}}\toprule
    Model & Algorithm & Jac-Norm & Spec-$L_1$ & Spec-Fro\\\hline
     \multirow{3}{*}{ResNet-110} & Vanilla & 17.7& $\infty$&$\infty$\\
         & Spectral (SN) & 17.8&10.8 &7.4\\
         & SRN-30 & {\bf 17.2}& {\bf 10.7} & {\bf 7.2}\\\cmidrule{2-5}
     \multirow{4}{*}{WideResNet-28-10} & Vanilla & 16.2& 14.60&11.18\\
         & Spectral (SN) & 16.13& 7.23&4.5\\
         & SRN-50 & 15.8& 7.3&4.5\\
         & SRN-30 & {\bf 15.7}& {\bf 7.20}&{\bf 4.4}\\\cmidrule{2-5}
     \multirow{4}{*}{Densenet-100} & Vanilla &19.2 &$\infty$ &$\infty$\\
         & Spectral (SN) &17.8 & 12.2&9.4\\
         & SRN-50 &17.6 &12 &9.2\\
         & SRN-30 & {\bf 17.7}&{\bf 11.8} &{\bf 9.0}\\\hline
  \end{tabular}
  \caption[Values of 90 percentile of $\log$ complexity measures
  from~\cref{fig:compl}]{Values of 90 percentile of $\log$ complexity measures
    from~\cref{fig:compl}. Here $\infty$ refers to the situations
    where the product of spectral norm blows up. This is the case in deep networks like ResNet-110 and Densenet-100 where the absence of spectral normalization (Vanilla)
    allows the product of spectral norm to grow arbitrarily large with an increasing number of layers. Lower is better.}
  \label{tab:perc-compl}
\end{table}
{\em The above experiments indicate that SRN, while providing enough capacity for the standard classification task, is remarkably less prone to memorisation and provides improved generalisation.}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


